Higher-Order Sinusoidal Input Describing Functions for Open-Loop and Closed-Loop Reset Control with Application to Mechatronics Systems

Reset control enhances the performance of high-precision mechatronics systems. This paper introduces a generalized reset feedback control structure that integrates a single reset-state reset controller, a shaping filter for tuning reset actions, and linear compensators arranged in series and parallel configurations with the reset controller. This structure offers greater tuning flexibility to optimize reset control performance. However, frequency-domain analysis for such systems remains underdeveloped. To address this gap, this study makes three key contributions: (1) developing Higher-Order Sinusoidal Input Describing Functions (HOSIDFs) for open-loop reset control systems; (2) deriving HOSIDFs for closed-loop reset control systems and establishing a connection with open-loop analysis; and (3) creating a MATLAB-based App to implement these methods, providing mechatronics engineers with a practical tool for reset control system design and analysis. The accuracy of the proposed methods is validated through simulations and experiments. Finally, the utility of the proposed methods is demonstrated through case studies that analyze and compare the performance of three controllers: a PID controller, a reset controller, and a shaped reset controller on a precision motion stage. Both analytical and experimental results demonstrate that the shaped reset controller provides higher tracking precision while reducing actuation forces, outperforming both the reset and PID controllers. These findings highlight the effectiveness of the proposed frequency-domain methods in analyzing and optimizing the performance of reset-controlled mechatronics systems.

==> 2_Problem_Statement.tex <==
\section{Motivation and Problems Statement}
\label{sec: problem statement}
This section outlines two main research problems addressed in this study: (1) Section \ref{subsec: open-loop problem} demonstrates the inaccuracies in previous open-loop frequency response analysis for reset control systems; (2) Section \ref{subsec: the closed-loop problem} illustrates the need for closed-loop frequency response analysis methods.
% and the necessity of two-reset condition for this analysis.
% (2) Section \ref{subsec: the need of avoid mrcs} discusses the necessity to avoid multiple-reset actions in closed-loop systems;
% Frequency response analysis is an effective tool in practical control system design. However, the inherent higher-order harmonics of reset control complicate this analysis. Currently, there is a lack of methods for both open-loop and closed-loop frequency response analysis of the reset control system shown in Fig. \ref{fig1:RC system}. This work aims to addresses this gap.
\subsection{Inaccuracy in Previous Open-Loop Frequency Response Analysis}
\label{subsec: open-loop problem}
% Frequency response provides essential magnitude and phase information of the system, which is essential for the control system design \cite{tian2007frequency}. It is obtained by analyzing the steady-state responses of reset control systems to sinusoidal inputs across varying frequencies. 
Figure \ref{fig: open_loop_rcs} depicts the block diagram of the open-loop reset control system.
 % In this configuration, the reset controller \(\mathcal{C}_r\) \eqref{eq: State-Space eq of RC} receives an input signal \(z_o(t) = |Z_o|\sin(\omega t + \angle Z_o)\) and generates an output signal \(m_o(t)\), assuming that Assumption \ref{assum: open-loop stability} is satisfied. The reset-triggered signal \(z_s(t)\) is defined as \(z_s(t) = |Z_o \mathcal{C}_s(\omega)|\sin(\omega t + \angle Z_o + \angle \mathcal{C}_s(\omega)\), which is obtained by filtering \(z_o(t)\) through the transfer function \(\mathcal{C}_s\).
\begin{figure}[H]
	%	\missingfigure{RCsystem} 
    \centering
         % \captionsetup{singlelinecheck = false, format= hang, justification=justified, font=footnotesize, labelsep=space}
           \centering
	\includegraphics[width=0.75\columnwidth]{figs/open_loop_rcs.pdf}
	\caption{Block diagram of the open-loop reset control system.}
	\label{fig: open_loop_rcs}
\end{figure}

% The Higher-Order Sinusoidal Input Describing Function (HOSIDF) is a technique used for analyzing the frequency response of nonlinear systems \cite{nuij2006higher}. Consider the reset controller \(\mathcal{C}_r\) in Fig.\ref{fig: open_loop_rcs} with a sinusoidal input signal \(z_o(t) = |Z_o|\sin(\omega t+\angle Z_o)\) and a shaping filter $\mathcal{C}_s$, satisfying the condition in \eqref{eq:open-loop stability}. Due to the nonlinearity in the system, the output signal \(m_o(t)\) consists of infinite harmonics, represented as \(m_o(t) = \sum\nolimits_{n=1}^{\infty} m_o^n(t), \ n\in\mathbb{Z}^+\), with the Fourier transform $M_o^n(\omega)$. The HOSIDF method employs a ``Virtual Harmonics Generator" (VHG) to generate \(n\) harmonics from the input signal \(z_o(t)\), formulated as \(z_o^n(t) = |Z_o|\sin(n\omega t+n\angle Z_o)\), with the Fourier transform $Z_o^n(\omega)$. Subsequently, the function \(\mathcal{C}_r^{n}(\omega)\) is defined as the transfer function from \(z_o^n(t)\) to \(m_o^n(t)\). Research \cite{karbasizadeh2022band} developed \(\mathcal{C}_r^{n}(\omega) = M_o^n(\omega)/Z_o^n(\omega)\) as given by
% \begin{equation}
% \label{eq: Hn} 
% % \resizebox{0.99\columnwidth}{!}{$
% \mathcal{C}_r^{n}(\omega)= 
%  \begin{cases}
%         C_R(A_R-j\omega I)^{-1}\Theta_\phi(\omega) +\mathcal{C}_l(\omega), & \text{for } n=1, \\
% 		C_R(A_R -j\omega nI)^{-1}\Theta_\phi(\omega), & \text{for odd }n>1, \\
% 		0,&\text{for even }n\geqslant 2 ,
%   \end{cases}
%   % $}
% \end{equation}
% where 
% \begin{equation}
% \begin{aligned}
%     \Theta_\phi(\omega) &= \frac{-2j\omega e^{j\angle \mathcal{C}_s(\omega)}}{\pi}\Omega(\omega)[\omega I \cos(\angle \mathcal{C}_s(\omega))
%     % \\    &\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \
%     -A_R\sin(\angle \mathcal{C}_s(\omega))]\Lambda^{-1}(\omega) B_R,\\
%     \Omega(\omega) &= \Delta(\omega) - \Delta(\omega){\Delta_r}^{-1}(\omega)A_\rho\Delta(\omega),\\
%     % \Theta _D(\omega) &= \frac{-2\omega ^2}{\pi}\Delta(\omega)[\Gamma _r(\omega)-\Lambda ^ {-1}(\omega)],\\
%    % \Gamma _r(\omega) &= \Delta _r^{-1}(\omega)A_{\rho}\Delta(\omega)\Lambda ^ {-1}(\omega),\\
%    \Delta _r(\omega) &= I+A_{\rho}e^{(\frac{\pi}{\omega}A_R)},\\
%    % \Lambda(\omega) &= \omega ^2I+{A_R}^2,\\
%    \Delta(\omega) &= I+e^{(\frac{\pi}{\omega}A_R)},\\
%    \Lambda(\omega) &= \omega ^2I+{A_R}^2.
% \end{aligned}           
% \end{equation} 

% Based on \eqref{eq: Hn}, the steady-state output of a reset controller $\mathcal{C}_r$ under a sinusoidal input $z_o(t) = |Z_o|\sin(\omega t+\angle Z_o)$ is given by
% \begin{equation}
% \label{eq: mo'}
% m_o(t) = \sum\nolimits_{n=1}^{\infty}|Z_o \mathcal{C}_r^{n}(\omega)|\sin(n\omega t+n\angle Z_o + \angle  \mathcal{C}_r^{n}(\omega)).
% \end{equation}
 
% However, this analysis has certain accuracy limitations, as demonstrated in the following example. 

% Consider a reset controller \(\mathcal{C}_r\) characterized by the following design parameters: the BLC \(\mathcal{C}_{l} ={30\pi}/{s} + 1\) with a reset value of \(\gamma = 0\), and the shaping filter defined as \(\mathcal{C}_s =({s}/{(30\pi)} + 1)/({s}/{6000\pi} + 1)\).

% Figure \ref{fig: mot_previous} illustrates the simulated output \( m_o(t) \) of the reset controller \(\mathcal{C}_r\) in response to a sinusoidal input signal \( z_o(t) = \sin(20\pi t) \), compared with the output predicted by \eqref{eq: mo'}. The results indicate that the HOSIDF method in \eqref{eq: Hn} does not accurately capture the performance of the reset controller.
% \begin{figure}[!t]
%     \centering
% 	%	\missingfigure{RCsystem}
%         % \captionsetup{singlelinecheck = false, format= hang, justification=justified, font=footnotesize, labelsep=space}
% 	\centerline{\includegraphics[width=0.75\columnwidth]{figs/mo_t.pdf}}
% 	\caption{The output signal $m_o(t)$ for the reset controller $\mathcal{C}_r$ under the sinusoidal input \( z_o(t) = \sin(20\pi t) \), obtained from simulation and prediction.}
% 	\label{fig: mot_previous}
% \end{figure}


Consider a system with the following design parameters: reset controller $\mathcal{C}_r$ is built on a BLC $\mathcal{C}_l = 30\pi/s$ with the reset value $\gamma = 0$, $\mathcal{C}_1 = (s/(150\pi))/(s/(3000\pi) +1)$, $\mathcal{C}_2 = 1$, $\mathcal{C}_s = 1/(s/5 +1)$, $\mathcal{C}_3 = 1/(s/(150\pi) +1)$, $\gamma = 0$, $\mathcal{P} = 6.615\times10^5/(83.57s^2+279.4s+5.837\times10^5)$. The output signal $y_o(t)$ of the system under a sinusoidal input signal $e_o(t) =\sin(8\pi t)$ obtained from the analysis method in \cite{karbasizadeh2022band} and simulation are shown in Fig. \ref{fig: yot_previous}.
\begin{figure}[!t]
    \centering
	%	\missingfigure{RCsystem}
        % \captionsetup{singlelinecheck = false, format= hang, justification=justified, font=footnotesize, labelsep=space}
	\centerline{\includegraphics[width=0.75\columnwidth]{figs/ex4_yo_Lo_previous.pdf}}
	\caption{The output signal $y_o(t)$ of the open-loop reset control system under the sinusoidal input \( e_o(t) =\sin(8\pi t)\), obtained from simulation and previous analysis.}
	\label{fig: yot_previous}
\end{figure}


The results in Fig. \ref{fig: yot_previous} show that the method in \cite{karbasizadeh2022band} does not accurately capture the performance of the reset control system. This inaccuracy stems from the method's failure to account for the influence of the shaping filter \(\mathcal{C}_s\) on the phase of high-order harmonics in the system, despite accurately calculating their magnitudes. As a result, the method is reliable only when \(\angle \mathcal{C}_s(s) = 0\) or when higher-order harmonics are sufficiently small to be neglected. However, both magnitude and phase information in frequency responses are crucial, particularly in closed-loop frequency response analysis, where the phases of higher-order harmonics in the open loop impact the behavior of each harmonic in the closed-loop system via the feedback loop.
% , as discussed below.

% A reset control system is designed with the following parameters: $\mathcal{C}_1 = 1/(s/5 +1)$, $\mathcal{C}_r = 30\pi/s$ with the reset value $\gamma = 0$, $\mathcal{C}_2 = 1$, $\mathcal{C}_s = (s +1)/(s/2 +1)$, $\mathcal{C}_3 = 1/(s/(150\pi) +1)$, $\gamma = 0$, $\mathcal{P} = 6.615e5/(83.57s^2+279.4s+5.837e5)$. The system is subject to a sinusoidal input signal $e_o(t)=\sin(10\pi t)$. 
% \begin{figure}[!t]
% 	%	\missingfigure{RCsystem}
%         \captionsetup{singlelinecheck = false, format= hang, justification=justified, font=footnotesize, labelsep=space}
% 	\centerline{\includegraphics[width=0.45\columnwidth]{figs/yot_example2_sim_oldpre.pdf}}
% 	\caption{The simulation and prediction of the open-loop output, denoted as \( y_o(t) \), for the reset control system under the sinusoidal input \( e_o(t) = \sin(10\pi t) \).}
% 	\label{fig: yot_example2_sim_oldpre}
% \end{figure}

% Figure \ref{fig: yot_example2_sim_oldpre} shows the simulated and predicted output \( y_o(t) \) of the open-loop reset control system, comparing the results from equation \eqref{eq: yo'}. The analysis demonstrates that the open-loop HOSIDF method described in \eqref{eq: Lo'} is inaccurate for evaluating this system.

% Currently, there is no precise analysis method for the open-loop reset control system depicted in Fig. \ref{fig: open_loop_rcs}. 

To correct this inaccuracy, Section \ref{sec: Toolbox 1} develops a new HOSIDF analysis method for the open-loop reset control system. This is achieved by extending the analysis theory applied to a specific class of reset control systems characterized by \(\mathcal{C}_1 = \mathcal{C}_s = \mathcal{C}_3 = \mathcal{C}_4 = 1\) and \(\mathcal{C}_2 = 0\) in our prior research \cite{ZHANG2024106063}, to the generalized reset control systems, as illustrated in Fig. \ref{fig: open_loop_rcs}.


% This inaccuracy arises from two errors: the first is the inaccurate calculation of the reset controller $\mathcal{C}_r$ in \eqref{eq: Hn}, and the second is the omission of the phase shift introduced by \(\mathcal{C}_1(s)\) on the higher-order harmonics in \eqref{eq: Lo'} for $n>1$. Both errors stem from the incorrect calculation of the phase effects between the signal $e_o(t)$ and the reset trigger signal $z_s(t)$. The second error was also addressed in research \cite{caporale2024practical}, but the method there is not applicable for reset control sytems with the shaping filter $\mathcal{C}_s$. 

% Moreover, by accounting for phase shifts and decomposing the output into linear and nonlinear components. Such decomposition supports more effective frequency-domain analysis for closed-loop reset control sytems.

% \subsection{Need of Identifying Multiple-Reset Actions in Sinusoidal-Input Closed-Loop reset control sytems}
% \label{subsec: the need of avoid mrcs}
% In sinusoidal-input frequency responses of closed-loop systems, two scenarios can arise: systems experiencing two resets per cycle (two-reset control sytems) and those undergoing multiple resets per cycle (multiple-reset control sytems). Current sinusoidal-input frequency response analysis methods \cite{saikumar2021loop,ZHANG2024106063} assume closed-loop reset control sytems are two-reset control sytems, leading to deviations in the analysis for multiple-reset control sytems. Thereby, to ensure accurate closed-loop frequency response analysis for reset control sytems, a tool for identifying multiple-reset control system regions in the working frequency is required. Furthermore, multiple-reset control sytems indicate high-magnitude higher-order harmonics, which can degrade performance and should be avoided \cite{ZHANG2024106063}.

% % Therefore, identifying multiple-reset actions in sinusoidal-input closed-loop reset control sytems is crucial to avoid them during system design.
% Previous literature \textcolor{red}{[cite J2]} proposes a method for identifying multiple-reset control sytems specifically in closed-loop reset control sytems, where \(\mathcal{C}_1 = \mathcal{C}_3 = \mathcal{C}_4 = 1\) and \(\mathcal{C}_2 = 0\). Section \ref{sec: Toolbox 2} extends this method to a broader generalized reset control structure in Fig. \ref{fig1:RC system}, equipping engineers with tools to design reset control sytems that mitigate multiple-reset actions.

% In sinusoidal-input frequency responses of open-loop reset control sytems, there are usually two reset instants per cycle. However, 
% In the closed-loop frequency response analysis, two scenarios can arise in sinusoidal-input reset control sytems: two-reset or multiple-reset instants per steady-state period, referred to as two-reset and multiple-reset control sytems, respectively. These multiple-reset actions present two primary challenges. First, there are no established frequency response analysis tools for such systems, and current methods, such as the DF analysis, are inaccurate for multiple-reset scenarios \textcolor{red}{[cite J2]}. Second, multiple-reset actions generate higher-order harmonics with significant magnitudes, which can adversely affect overall system performance. These issues have been exclusively discussed in our previous research \textcolor{red}{[cite J2]}.




% \begin{figure}[!t]
%     \centering
%     \captionsetup{singlelinecheck = false, format= hang, justification=justified, font=footnotesize, labelsep=space}
%     \includegraphics[width= 0.9\columnwidth]{figs/MRC_examples_sin5Hz_100Hz.pdf}
%     \caption{The reset-triggered signal \(z_s(t)\) of the system is analyzed under input signals: ($a_1$) \(r(t) = \sin(10\pi t)\) and ($b_1$) \(r(t) = \sin(200\pi t)\), with reset instants marked by blue circles. The PSD analysis of the steady-state errors for both scenarios is presented in ($a_2$) and ($b_2$).}
% 	\label{fig:MRC_examples_sin1Hz_100Hz}
% \end{figure}
% To illustrate the two problems raised by multiple-reset actions, we apply a reset control system shown in Fig. \ref{fig1:RC system} with the following parameters: \(\mathcal{C}_1(s) = {(s/(150\pi) + 1)}/{(s/(3000\pi) + 1)}\), \(\mathcal{C}_s(s) = {1}/{(s/(1500\pi) + 1)}\), \(\mathcal{C}_r = {(30\pi)}/{s}\), \(\mathcal{C}_2(s) = 1\), \(\mathcal{C}_3(s) = 20.5 /{(s/(150\pi) + 1)} \cdot {(s/(62.5\pi) + 1)}/{(s/(1440\pi) + 1)} \cdot {(1+15\pi/s)} \cdot {1}/{(s/(3000\pi) + 1)}\), $\gamma = 0$, and \(\mathcal{P}(s) = {6.615e5}/{(83.57s^2 + 279.4s + 5.837e5)}\).

% Figure \ref{fig:MRC_examples_sin1Hz_100Hz}($a_1$) and ($b_1$) illustrate the reset-triggered signal \(z_s(t)\) of the system under input signals \(r(t) = \sin(10\pi t)\) and \(r(t) = \sin(200\pi t)\), respectively. At input frequencies of 1 Hz and 100 Hz, the system experiences multiple-reset actions and two-reset actions, respectively.

% The Power Spectral Density (PSD) analysis of the steady-state errors for these two systems is shown in Fig. \ref{fig:MRC_examples_sin1Hz_100Hz}($a_2$) and ($b_2$). In systems with multiple-reset actions, the higher-order harmonics are significant, whereas in two-reset control systems, the higher-order harmonics are relatively minor and can be considered negligible.
% This is the objective of designing reset control systems: to take advantage of the benefits of the first-order harmonics and minimize the effects of higher-order harmonics.
\subsection{Need of Frequency Response Analysis for Closed-Loop Reset Control Systems}
\label{subsec: the closed-loop problem}
In addition to open-loop analysis, closed-loop frequency response analysis is crucial for designing reset control sytems and applying loop-shaping techniques. For example, in linear systems, using the SIDF analysis, the sensitivity function is given by
\begin{equation}
\label{eq: S_linear}
   \mathcal{S}(\omega) = \frac{1}{1+\mathcal{L}(\omega)},
\end{equation}
where $\mathcal{L}(\omega)$ is the open-loop transfer function of the linear system. The sensitivity function \(\mathcal{S}(\omega)\) in \eqref{eq: S_linear} characterizes the connection between the closed-loop system and the open-loop transfer function \(\mathcal{L}(\omega)\). It also provides insights into the system’s steady-state errors and evaluates the modulus margin, which serves as an indicator of the system’s robustness to variations in gain or phase within the control loop \cite{schmidt2020design}.
% Furthermore, the sensitivity function relates directly to the **steady-state error** of the system, which is the difference between the desired and actual output as time approaches infinity. Lower values of \(\mathcal{S}(\omega)\) at low frequencies indicate improved steady-state performance, as they reflect the system's ability to minimize residual error. Thus, the sensitivity function is instrumental in designing and analyzing feedback systems, as it balances robustness, transient performance, and steady-state accuracy, helping engineers optimize control strategies for reliable and responsive systems.

Nevertheless, the interaction between first-order and higher-order harmonics within the closed-loop structure introduces cross-effects, making the open-loop and closed-loop relation in \eqref{eq: S_linear} does not hold.  Currently, there are no established frequency response analysis methods for the generalized closed-loop reset control systems depicted in Fig. \ref{fig1:RC system}. To overcome this limitation, this work extends the HOSIDF framework—originally developed for a specific configuration where \(\mathcal{C}_1 = \mathcal{C}_s = \mathcal{C}_3 = \mathcal{C}_4 = 1\) and \(\mathcal{C}_2 = 0\) \cite{ZHANG2024106063}—to accommodate the generalized reset control structure illustrated in Fig. \ref{fig1:RC system}.

In the sinusoidal-input frequency response analysis of closed-loop systems, two scenarios arise: two-reset control systems, which undergo two resets per steady-state cycle, and multiple-reset control systems, which experience more than two resets per cycle. Multiple-reset actions typically indicate high-magnitude higher-order harmonics that can degrade performance and should thus be avoided \cite{ZHANG2024106063}. Additionally, current closed-loop SIDF analysis methods for reset control systems commonly assume two-reset systems \cite{saikumar2021loop,van2024higher}. To address this, the closed-loop reset control system is initially configured to operate as a two-reset control system by ensuring it satisfies the two-reset condition outlined in \cite{Xinxin_multiple_reset}. Once this condition is met, the closed-loop HOSIDFs developed in this study—encompassing the sensitivity function, complementary sensitivity function, and control sensitivity function for each harmonic—are applied to analyze the system dynamics.
% In the frequency response analysis of closed-loop systems subjected to sinusoidal inputs, two scenarios may occur: systems that experience two resets per cycle (referred to as two-reset control systems) and those that undergo multiple resets per cycle (referred to as multiple-reset control systems). Current methods for sinusoidal-input frequency response analysis \cite{saikumar2021loop,ZHANG2024106063} typically assume that closed-loop reset control systems operate as two-reset control systems. This assumption will lead to inaccuracies in the analysis for multiple-reset control systems. To ensure accurate closed-loop frequency response analysis for reset control systems, it is essential to establish a two-reset condition. Furthermore, multiple-reset actions in sinusoidal-input reset control systems indicate the presence of high-magnitude high-order harmonics, which can negatively impact performance and should be avoided \cite{ZHANG2024106063}. Therefore, prior to conducting closed-loop analysis, a two-reset condition is employed to prevent multiple-reset actions.

% Previous literature \textcolor{red}{[cite J2]} proposes a two-reset condition specifically for reset control systems with \(\mathcal{C}_1 = \mathcal{C}_3 = \mathcal{C}_4 = 1\) and \(\mathcal{C}_2 = 0\). Section \ref{sec: Toolbox 2} extends this method to encompass a broader generalized reset control structure in Fig. \ref{fig1:RC system}, thereby providing engineers with tools to design reset control systems that effectively mitigate multiple-reset actions.

% , $W(\omega)$ ($Z^n(\omega)$), $e_s(\omega)$ ($e_s^n(\omega)$), $M(\omega)$ ($M^n(\omega)$), $V(\omega)$ ($V^n(\omega)$), $U(\omega)$ ($U^n(\omega)$), and $Y(\omega)$ ($y^n(\omega)$). 

% Note that the closed-loop two-reset control system is designed based on the multiple-reset identification tool.
% The three contributions in Sections \ref{sec: Toolbox 1} to \ref{sec: Toolbox 3} are integrated into MATLAB toolboxes. Simulations and experiments conducted on the precision motion stage in Fig. \ref{fig1:Spyder} validate the effectiveness of the proposed methods.

% \subsection{Higher-Order Sinusoidal Input Describing Function (HOSIDF) for Reset Controller $\mathcal{C}_r$}
% \begin{prop}(\cite{nuij2006higher, heinen2018frequency, dastjerdi2022closed, karbasizadeh2022band})
% \label{prop: Cr_Hn}
% In the open-loop SISO controller $\mathcal{C}_r$ described in \eqref{eq: Hn}, where the input signal is denoted as $z(t) = |W|\sin(\omega t)$, a reset signal is defined as $z_s(t) = |W|\cdot|\mathcal{C}_s(\omega)|\sin(\omega t + \angle\mathcal{C}_s(\omega))$. To analyse this system, a method referred to as the \enquote{Virtual Harmonics Generator} is employed to define the HOSIDF. This HOSIDF $\mathcal{H}^n(\omega)$, serves to characterise the transfer function from the input signal $z(t)$ to the output signal $m(t)$. The expression for $\mathcal{H}^n(\omega)$ can be formulated as:
% \begin{equation}
% 	\label{eq: Hn} 
% 	\mathcal{H}^n(\omega)= \begin{cases}
%         C_R(A_R-j\omega I)^{-1}\Theta_\phi(\omega) +\\C_R(j\omega I-A_R)^{-1}B_R+D_R, & n=1 \\
% 		C_R(A_R -j\omega nI)^{-1}\Theta_\phi(\omega), & \text{odd }n>2 \\
% 		0,&\text{even }\geqslant 2 ,
%   \end{cases}
% \end{equation}
% where 
% \begin{equation}
% \begin{aligned}
%     \Theta_\phi(\omega) &= \frac{-2j\omega e^{j\angle \mathcal{C}_s(\omega)}}{\pi}\Omega(\omega)[\omega I \cos(\angle \mathcal{C}_s(\omega))\\
%     &\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \
%     -A_R\sin(\angle \mathcal{C}_s(\omega))]\Lambda^{-1}(\omega) B_R,\\
%     \Omega(\omega) &= \Delta(\omega) - \Delta(\omega){\Delta_r}^{-1}(\omega)A_\rho\Delta(\omega),\\
%     % \Theta _D(\omega) &= \frac{-2\omega ^2}{\pi}\Delta(\omega)[\Gamma _r(\omega)-\Lambda ^ {-1}(\omega)],\\
%    % \Gamma _r(\omega) &= \Delta _r^{-1}(\omega)A_{\rho}\Delta(\omega)\Lambda ^ {-1}(\omega),\\
%    \Delta _r(\omega) &= I+A_{\rho}e^{(\frac{\pi}{\omega}A_R)},\\
%    % \Lambda(\omega) &= \omega ^2I+{A_R}^2,\\
%    \Delta(\omega) &= I+e^{(\frac{\pi}{\omega}A_R)},\\
%    \Lambda(\omega) &= \omega ^2I+{A_R}^2.
% \end{aligned}      
% \end{equation}    
% \end{prop}
% [\textcolor{teal}{Tested}]

% In the case where $\mathcal{C}_s(\omega)=1$, $\mathcal{H}^n(\omega)$ corresponds to the HOISDF in previous works such as \cite{saikumar2021loop, heinen2018frequency}. Additionally, $H^1(\omega)$ corresponds to the conventional DF analysis used for RCSs as described in \cite{guo2009frequency}.

%In the frequency domain, the response of reset controllers could be roughly analyzed by sinusoidal input DF. However, DF only encompasses the first harmonic of the Fourier series expansion of reset output $u_R(t)$ in Fig. \ref{fig1:RC system}, whereas there are infinite higher harmonics in $u_R(t)$. Therefore, there will be large deviations if DF is applied to estimate the behavior of the reset controller. To decrease the analysis error caused by DF, a virtual harmonic generator \cite{nuij2006higher}, is introduced to extend the DF to the HOSIDF as shown in Fig. \ref{fig:HOSIDF}. The given reset input signal $e(t)=A\sin (\omega t)$ goes through the virtual harmonic generator and then generates parallel harmonics with varying magnitudes and phases, enabling higher-order harmonics analysis. When the number of harmonics is 1, the HOSIDF is exactly the DF. In HOSIDF, 

% \subsection{Problem Formulation}
% Frequency-domain analysis is an invaluable approach for the analysis of control systems in industrial applications. Currently, there is a lack of an accurate  frequency-domain analysis method applicable to both open-loop and closed-loop RCSs in Fig. \ref{fig1:RC system}. Thus, we elaborate on the research problems addressed in this paper in Problem \ref{prob1}, \ref{prob2}, and \ref{prob3}.
% \begin{prob}
% \label{prob1}
% Develop a open-loop HOSIDF for a SISO RCS in Fig. \ref{fig1:RC system} under sinusoidal inputs.
% \end{prob}
% \begin{prob}
% \label{prob2}
% Develop a closed-loop HOSIDF for a SISO RCS in Fig. \ref{fig1:RC system} under sinusoidal inputs.
% \end{prob}
% \begin{prob}
% \label{prob3}
% Connect the open-loop and closed-loop analysis together and establish a comprehensive frequency-domain design methodology for RCSs, which can be readily applied in industrial settings.
% \end{prob}
% \subsection{Fundamental Definitions}
% This subsection presents definitions and notations used through the whole paper.
% \begin{defn} 
% \end{defn}
% \begin{defn}
% The uppercase format of a variable signifies its Fourier transform. To illustrate, $E_{l}(\omega)$, $U_{l}(\omega)$, and $Y_{l}(\omega)$ correspond to the Fourier transforms of $e_{l}(t)$, $u_{l}(t)$, and $y_{l}(t)$, respectively. Similarly, we define $R(\omega)$, $E(\omega)$, $U(\omega)$, and $Y(\omega)$ as the Fourier transforms of $r(t)$, $e(t)$, $u(t)$, and $y(t)$, respectively.
% \end{defn}

%\subsection{Reset Elements}
%This part presents the current most popular reset elements and their DF representatives, including Clegg integrator (CI) and First-order reset element (FORE).  
%\subsubsection{Generalized Clegg Integrator (GCI)}
%The simplest reset element clegg integrator (CI) is firstly proposed in 1958 \cite{clegg1958nonlinear}. The mechanism of CI is that when the input signal hits zero, the integral output resets to zero. The CI was then extended to the Generalized Clegg Integrator (GCI) that the after-reset value is defined to be a proportional value of its base-linear output.
%The state-space matrices of GCI based on \eqref{eq: Hn} are given as below. 
%\begin{equation}
%	A_R = 0,\ B_R = 1,\ C_R = 1,\ D_R = 0, A_\rho = \gamma \in [-1,1]. 
%\end{equation}
%% Its transfer function can be depicted as
%%\begin{equation} 
%%	\label{eq:GCI}
%%	G_{CI} = \frac{1}{\cancelto{}{s}\ \gamma},
%%\end{equation}
%%where the range of $\gamma$ is [-1,1].
%%where $\alpha$ compensates for the change of DF gain with respect to frequency response of linear integrator $\frac{1}{\alpha s}$. It has been proved that when $\gamma = 0$, $\alpha = 1.62$, and $\alpha$ varies as the reset value $\gamma$ changes \cite{saikumar2019constant}. 
%
%\subsubsection{Generalized FORE (GFORE)}
%First-order reset element (FORE) was originally reported in \cite{horowitz1975non}, and then was developed to the Generalized FORE (GFORE) \cite{guo2009frequency}. The base-linear counterpart of GFORE is the first-order low-pass filter. 
%The state-space representatives of GFORE are given as
%\begin{equation}
%	A_R = -\omega_r,\ B_R = \omega_r,\ C_R = 1,\ D_R = 0, A_\rho = \gamma \in [-1,1].
%\end{equation}
%Similarly, the Second-order reset element (SORE) is the second-order low-pass filter encapsulating the reset law.
%The transfer function of GFORE with a corner frequency at $\omega_r$ are 
%\begin{equation} 
%	\label{eq:GFORE}
%	G_{FORE} = \frac{1}{\cancelto{}{\frac{s}{\omega_r}}\ \gamma +1}.
%\end{equation}
%%where $\alpha$ corrects for the change of DF gain at high frequencies, which depends on the reset value $\gamma$. 
%\subsubsection{‘Constant in gain Lead in phase’ (CgLp)}
%The ‘Constant in gain Lead in phase’ (CgLp) element is firstly presented in \cite{saikumar2019constant}, which is designed by constructing a FORE or SORE with corresponding first- or second-order linear lead elements, respectively. When the corner frequency of FORE or SORE is $\omega_r$, the zero and pole of their following lead elements locate at $\omega_r$  and $\omega_f\ (\omega_f \gg \omega_r)$. The transfer function of first-order CgLp combining FORE and first-order lead filter is defined as
%\begin{equation} 
%	\label{eq:GCgLp}
%	G_{CgLp} = \left(\frac{1}{\cancelto{}{\frac{s}{\alpha \omega_r}}\ \gamma+1}\right)\left(\frac{\frac{s}{\omega_r}+1}{\frac{s}{\omega_f}+1}\right),
%\end{equation}
%where $\alpha$ compensates for the change of DF gain to the frequency response of the FORE.\\
%The state-space matrices of first-order CgLp are 
%\begin{equation}
%	\begin{aligned}
%		A_R = 
%		\begin{bmatrix}
%			-\alpha \omega_r & 0\\
%			\omega_f & -\omega_f
%		\end{bmatrix},
%		\ B_R =
%		\begin{bmatrix}
%			\alpha \omega_r \\
%			0
%		\end{bmatrix},\\
%		C_R=
%		\begin{bmatrix}
%			\frac{\omega_f}{\omega_r} & {1-\frac{\omega_f}{\omega_r}}
%		\end{bmatrix},
%		\ D_R=0, 
%		\ A_{\rho} = 
%		\begin{bmatrix}
%			\gamma & 0\\
%			0 & 1
%		\end{bmatrix}.
%	\end{aligned}
%\end{equation}
%CgLp advances in providing notable phase lag reduction in the range $[\omega_r,\omega_f]$ without sacrificing the gain profile in terms of DF analysis, which has the benefit of broadband phase compensation. Besides, it has more tuning freedoms and is easy to fit into the PID framework.
%\textcolor{red}{Be careful and accurate.}


==> Other.tex <==
\subsection{RC}

The reset elements have been used in a variety of applications, including motion control, robotics, power electronics, and aerospace engineering. The key advantages of reset control include its ability to handle highly nonlinear systems, its insensitivity to modeling errors and parameter uncertainties, and its improved disturbance rejection capabilities.


This method is particularly effective for rejecting narrow-band disturbances that can be well characterised in the frequency domain. Various techniques such as notch filters, lead-lag compensators, and proportional-integral-derivative (PID) controllers can be used to design a compensator that can reject disturbances at specific frequencies.

\subsection{Frequency-domain analysis}

Through assessing the system's response to different input frequencies and identifying critical frequency ranges that ma lead to instability or performance degradation, one can a compensator that introduces supplementary phase shift and gain. This serves to dampen disturbances at targeted frequencies.


Frequency domain analysis methods provide a powerful framework for analyzing control systems in the motion control field. These methods involve the examination of system behaviour and performance in the frequency domain, where signals and system responses are decomposed into their constituent frequency components. This allows engineers to assess the system's response to different input frequencies and identify critical frequency ranges that may lead to instability or performance degradation. One of the key tools in frequency domain analysis is the frequency response function, which characterizes how a system responds to sinusoidal inputs at different frequencies. By analyzing the magnitude and phase response of the frequency response function, engineers can evaluate important system properties such as gain, resonance frequencies, and phase shift. This information is crucial for understanding system stability, bandwidth requirements, and control system design. Furthermore, frequency domain analysis methods enable engineers to investigate the effects of disturbances and noise on the system performance. By examining the system's frequency response to disturbances, engineers can assess the system's robustness and design appropriate control strategies to mitigate the effects of disturbances. 

In addition to assessing system performance, frequency domain analysis methods also aid in control system design and optimization. Techniques such as loop shaping, gain and phase margin analysis, and controller tuning methods can be employed to achieve desired system performance specifications. Engineers can manipulate the frequency response characteristics to improve stability, reduce oscillations, and enhance control system performance. Overall, frequency domain analysis methods provide a comprehensive understanding of control systems in the motion control field. By leveraging the insights gained from frequency domain analysis, engineers can design and optimize control systems to meet the stringent requirements of high-performance motion control applications. 

\subsection{Other Control}
Robust Control: Robust control methods are designed to ensure stability and performance in the presence of uncertainties and variations in system parameters. These methods often use techniques like H-infinity control to provide robust disturbance rejection.

Model Predictive Control (MPC): MPC is an advanced control strategy that predicts the future behavior of a system and computes control actions based on optimizing a cost function. MPC is effective for handling disturbances and constraints in complex systems.

Sliding Mode Control: Sliding mode control aims to make the system's state converge to a predefined sliding surface. This control strategy is robust to disturbances and uncertainties and can provide fast response times.

Fractional Order Control: 

Model Predictive Control (MPC) is a powerful control strategy that has gained popularity in various fields due to its ability to handle complex systems and constraints. However, there are certain reasons why MPC might not be as widely used in industrial motion control applications:

Computation Complexity: MPC involves solving optimization problems at each control interval to determine the optimal control actions. This can  especially for systems with fast dynamics, high sampling rates, and complex constraints. Real-time implementation of MPC can be challenging in systems that require rapid control updates.

Prediction Horizon: MPC relies on predicting the future behavior of the system and optimizing control actions accordingly. The choice of prediction horizon affects the trade-off between stability and performance. Selecting an appropriate prediction horizon can be difficult, and a longer prediction horizon may lead to increased computational demands.

Tuning and Implementation: Designing an MPC controller requires accurate system models and careful tuning of various parameters, including prediction horizon, control weights, and constraints. Implementing an MPC controller in an industrial setting may require specialized knowledge and resources for model identification and tuning.

Nonlinearity and Complexity: Industrial motion control systems often exhibit nonlinearity, friction, backlash, and other complex behaviors that can challenge the accuracy of predictive models used in MPC. Handling such complexities requires accurate model identification and validation.

Robustness and Uncertainty: Industrial environments are subject to uncertainties, disturbances, and parameter variations. Ensuring the robustness of an MPC controller against such uncertainties requires additional efforts in terms of modeling, estimation, and control design.

Sampling Rates: Industrial motion control systems often operate at high speeds with tight control loops. The inherent delay introduced by the MPC optimization process can limit its effectiveness in fast systems, where control actions need to be executed quickly.

Implementation Challenges: Implementing MPC in real-time control systems requires efficient algorithms and hardware. Industrial motion control systems often use specialized controllers and hardware platforms optimized for real-time performance, and integrating MPC into such systems can be challenging.

Despite these challenges, there are ongoing research efforts to adapt and enhance MPC for industrial motion control applications. Researchers and practitioners are working on developing more efficient optimization algorithms, addressing robustness and uncertainty issues, and finding ways to integrate MPC with existing industrial control platforms. As technology advances and computational resources become more powerful, the adoption of MPC in industrial motion control may increase, especially for applications where its benefits in terms of performance and constraint handling outweigh its challenges.





==> suggested_reviewer.tex <==
Aleksei Tepljakov aleksei.tepljakov@taltech.ee
Kai Wulff kai.wulff@tu-ilmenau.de
christoph.weise christoph.weise@tu-ilmenau.de
Inés Tejado Balsera itejbal@unex.es
Eduard Petlenkov eduard.petlenkov@taltech.ee
Clara-Mihaela Ionescu ClaraMihaela.Ionescu@UGent.be


Even though the paper include the theoretical, but it apply to the industrial.

Graphical abstract:
